Partial Quantifier Elimination

We consider the problem of Partial Quantifier Elimination (PQE). Given formula exists(X)[F(X,Y) & G(X,Y)], where F, G are in conjunctive normal form, the PQE problem is to find a formula F*(Y) such that F* & exists(X)[G] is logically equivalent to exists(X)[F & G]. We solve the PQE problem by generating and adding to F clauses over the free variables that make the clauses of F with quantified variables redundant. The traditional Quantifier Elimination problem (QE) is a special case of PQE where G is empty so all clauses of the input formula with quantified variables need to be made redundant. The importance of PQE is twofold. First, many problems are more naturally formulated in terms of PQE rather than QE. Second, in many cases PQE can be solved more efficiently than QE. We describe a PQE algorithm based on the machinery of dependency sequents and give experimental results showing the promise of PQE.

==> f2ootnote.tex <==
Notice that this definition does not rule out the possibility
that there is a clause implied by $H$ (that is not in $H$) that is
also implied by $G$.  In this case $H$ contains a ``hidden'' noise. So
one can come with other, more rigorous definitions of a noise-free
solution to the PQE problem.


==> m1erge.fig.tex <==
%
% merge procedure
%
\setlength{\intextsep}{4pt}
\setlength{\textfloatsep}{10pt}
%\begin{wrapfigure}{L}{2in}
\begin{figure}
%\begin{center}
\small
%\normalsize
\vspace{-10pt}
\begin{tabbing}
aaa\=bb\= cc\= ddddddd\= \kill
$\mi{merge}(\Phi,\pnt{q},v,\Sub{\DS}{asym},\DS,C_b,C_{\overline{b}})$\{\\
\tb{\scriptsize{1}}\> $\DS := \mi{join\_Dseqs\_of\_old\_clauses}(v,\Sub{\DS}{asym},\DS)$; \\
\tb{\scriptsize{2}}\> $\DS := \mi{update\_Dseqs\_of\_new\_clauses}(v,\DS)$; \\
\tb{\scriptsize{3}}\> if ($v \not\in X$) return(\DS); \\
\tb{\scriptsize{4}}\> if ($C_b \neq nil$)  $\DS := \DS \cup \{\mi{Dseq}(C_b)\}$;\\  
\tb{\scriptsize{5*}}\> if ($C_{\overline{b}} \neq nil$)  $\DS := \DS \cup \{\mi{Dseq}(C_{\overline{b}})\}$;\\  
\tb{\scriptsize{6}}\> return(\DS);\} \\
\end{tabbing} 
\vspace{-20pt}
\caption{\ti{merge} procedure}
\label{fig:merge}
\end{figure}
%\end{wrapfigure}

